Non-native Quantum Generative Optimization with Adversarial Autoencoders

Large-scale optimization problems are prevalent in several fields, including engineering, finance, and logistics. However, most optimization problems cannot be efficiently encoded onto a physical system because the existing quantum samplers have too few qubits. Another typical limiting factor is that the optimization constraints are not compatible with the native cost Hamiltonian. This work presents a new approach to address these challenges. We introduce the adversarial quantum autoencoder model (AQAM) that can be used to map large-scale optimization problems onto existing quantum samplers while simultaneously optimizing the problem through latent quantum-enhanced Boltzmann sampling. We demonstrate the AQAM on a neutral atom sampler, and showcase the model by optimizing 64px by 64px unit cells that represent a broad-angle filter metasurface applicable to improving the coherence of neutral atom devices. Using 12-atom simulations, we demonstrate that the AQAM achieves a lower Renyi divergence and a larger spectral gap when compared to classical Markov Chain Monte Carlo samplers. Our work paves the way to more efficient mapping of conventional optimization problems into existing quantum samplers.

==> figures/gen_model.tex <==

\begin{tikzpicture}[
roundnode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
]
    \node[roundnode]      (maintopic)                              {2};
\end{tikzpicture}

==> old_main/ifEnergy.tex <==

To use latent quantum-enhanced MCMC for optimization, we correlate the energy of samples generated by the latent Boltzmann distribution $E(\z)$ with the efficiency of samples in the problem data distribution $Y(\x)$ such that $-E(\z) \approx Y(p(\x \vert \z))$.
Then, if the prior $p(\z)$ is a Boltzmann distribution, sampling $p(\z) \propto -E(\z) \approx Y(p(\x \vert \z)) $ will generate samples $\x \sim p(\x \vert \z)$ Boltzmann distributed according to $p(\x) \propto e^{Y(\x)/\tau}/Z$.


==> old_main/scrap.tex <==

\begin{table}[htp]
\centering
\begin{tabular}{lcc}
\hline
\textbf{Layer} & \textbf{Output Shape} & \textbf{Param \#} \\
\hline
\quad Reshape& [4, 1, 32, 32] & -- \\
\quad Conv2d & [4, 32, 32, 32] & 320 \\
\quad SiLU & [4, 32, 32, 32] & -- \\
\quad ResnetBlock & [4, 32, 32, 32] & 19,616 \\
\quad MaxPool2d & [4, 32, 16, 16] & -- \\
\quad ResnetBlock & [4, 32, 16, 16] & 19,616 \\
\quad MaxPool2d & [4, 32, 8, 8] & -- \\
\quad ResnetBlock & [4, 32, 8, 8] & 19,616 \\
\quad AttnBlock & [4, 32, 8, 8] & 4,288 \\
\quad ResnetBlock & [4, 32, 8, 8] & 19,616 \\
\quad MaxPool2d & [4, 32, 4, 4] & -- \\
\quad ResnetBlock & [4, 32, 4, 4] & 19,616 \\
\quad AttnBlock & [4, 32, 4, 4] & 4,288 \\
\quad ResnetBlock & [4, 32, 4, 4] & 19,616 \\
\quad Conv2d & [4, 2, 4, 4] & 66 \\
\quad Flatten & [4, 32] & -- \\
\quad Linear & [4, 12] & 396 \\
\quad Tanh & [4, 12] & -- \\
\quad Quantizer & [4, 12] & -- \\
\hline
\textbf{Total params:} & & 127,054 \\
\textbf{Trainable params:} & & 127,054 \\
\textbf{Non-trainable params:} & & 0 \\
\textbf{Total mult-adds (M):} & & 114.92 \\
\hline
\textbf{Input size (MB):} & & 0.02 \\
\textbf{Forward/backward pass size (MB):} & & 8.83 \\
\textbf{Params size (MB):} & & 0.51 \\
\textbf{Estimated Total Size (MB):} & & 9.36 \\
\hline
\end{tabular}
\caption{Model Summary of Encoder}
\label{table:encoder_summary}
\end{table}

\section{Decoder Architecture}
\begin{table}[htbp]
\centering
\begin{tabular}{lcc}
\hline
\textbf{Layer (type:depth-idx)} & \textbf{Output Shape} & \textbf{Param \#} \\
\hline
Linear& [1, 32] & 416 \\
Unflatten& [1, 2, 4, 4] & -- \\
Conv2d& [1, 32, 4, 4] & 96 \\
ResnetBlock& [1, 32, 4, 4] & 19,616 \\
AttnBlock& [1, 32, 4, 4] & 4,288 \\
ResnetBlock& [1, 32, 4, 4] & 19,616 \\
ConvTranspose2d& [1, 32, 8, 8] & 4,128 \\
ResnetBlock& [1, 32, 8, 8] & 19,616 \\
AttnBlock& [1, 32, 8, 8] & 4,288 \\
ResnetBlock& [1, 32, 8, 8] & 19,616 \\
ConvTranspose2d& [1, 32, 16, 16] & 4,128 \\
ResnetBlock& [1, 32, 16, 16] & 19,616 \\
ConvTranspose2d& [1, 32, 32, 32] & 4,128 \\
ResnetBlock& [1, 32, 32, 32] & 19,616 \\
Conv2d& [1, 1, 32, 32] & 33 \\
Sigmoid& [1, 1, 32, 32] & -- \\
Reshape& [1, 1, 32, 32] & -- \\
\hline
\textbf{Total params:} & & 139,201 \\
\textbf{Trainable params:} & & 139,201 \\
\textbf{Non-trainable params:} & & 0 \\
\textbf{Total mult-adds (M):} & & 33.99 \\
\hline
\textbf{Input size (MB):} & & 0.00 \\
\textbf{Forward/backward pass size (MB):} & & 2.30 \\
\textbf{Params size (MB):} & & 0.56 \\
\textbf{Estimated Total Size (MB):} & & 2.86 \\
\hline
\end{tabular}
\caption{Model Summary of Decoder}
\label{table:decoder_summary}
\end{table}
\begin{equation}
    \mathbb{E}_{z\sim \tilde q_\phi(z|\chi)} \log[p_\theta(\chi|z)]
\end{equation}
    
\begin{equation}
    \mathbb{E}_{z\sim q_\phi(z|\chi)} \log[\tilde p_\theta(\chi|z')]
\end{equation}



$q_\phi(z|\chi) = \sum_{z'} R(z|z')\tilde q_\phi(z|\chi)=\sum_\epsilon \tilde q_\phi(z+\epsilon | \chi) P(\epsilon|z)$

$p_\theta(\chi|z) = \sum_{z'} R(z'|z)\tilde p_\theta(\chi|z) = \sum_\epsilon \tilde p_\theta(\chi | z + \epsilon) P(\epsilon | z )$
\begin{figure}
  \begin{center}
    \includegraphics[width=0.95\columnwidth]{./figures/pdf/full_ml_framework_column.pdf}
  \end{center}
  \caption{{\bf Adversarial quantum autoencoder models with a latent MCMC chain realize a Boltzmann prior.} A data sample $\x \sim p(\x)$ is encoded into an initial state $\z_0 \in \{0, 1\}^n$ using a variational attention network $q_\th(\z_0 \vert \x)$. The state is evolved using an adversarial channel $P(\z_{t+1} \vert \z_{t})$ that produces adversarial noise $\epsilon$ such that $\z_{t+1} = \epsilon + \z_t$. 
  Finally, the decoder reconstructs the input data using the final state $\z_f$ of the adversarial channel.  }
  \label{fig:auto}
\end{figure}
\begin{figure}
  \begin{center}
    \includegraphics[width=0.8\columnwidth]{./figures/pdf/total_volume.pdf}
  \end{center}
  \caption{\textbf{MCMC Metric Space} displays volumes of non-native samples with a Hamming distance metric. Each native sample is enclosed by a volume of samples reachable by a MCMC walk with 10 proposal steps of a given sampler. An example quantum MCMC volume displayed in red has a Hamming radius of $r=7$ for temperature $\tau=1000$ and $r=4$ for $\tau = 0.001$. This volume overlaps with a neighbor volume encoded in blue. For the local sampler volumes, the red and blue volumes do not overlap and have smaller Hamming radii. }
  \label{fig:auto}
\end{figure}
\subsection{Adversarial Quantum Autoencoder Model}



\subsection{Channel Capacity}
The channel capacity of the MCMC chain is defined as 
\begin{align}
    \sup_{q_\ph(\z_0 \vert \x)}\text{KL}(p(\z_f ; \z_0) \vert q_\ph(\z_0 \vert \x) p(\z_f \vert \x))
\end{align}
\begin{align}
    &\text{KL}(p(\z_f ; \z_0) \vert q_\ph(\z_0 \vert \x) p(\z_f \vert \x)) \nonumber \\
    &= \mathbb{E}_{(\z_f, \z_0) \sim p(\z_f ; \z_0)}\left[\log {\frac{p(\z_f ; \z_0)}{q_\ph(\z_0 \vert \x) p(\z_f \vert \x))}}\right] \\
    &= \mathbb{E}_{(\z_f, \z_0) \sim p(\z_f ; \z_0)}\left[\log {\frac{p(\z_f \vert \z_0)p(\z_0)}{q_\ph(\z_0 \vert \x) p(\z_f \vert \x))}}\right]
\end{align}
\begin{align}
    \sup_{p(\z_f)}\text{KL}(p(\x ; \z_f) \vert p(\x) p(\z_f))
\end{align}
which can be upper bounded using previous approximating distributions as 
\begin{align}
    \sum_{\x \sim p(\x), \z_f \sim q_\ph(\z_f \vert \x)} p(\z_f; \x) \log \frac{ p(\z_f; \x) }{q_\ph(\z_f \vert \x) p_\th(\x \vert \z_f))} 
\end{align}
\begin{align}
    \mathbb{E}_{\x \sim p(\x), \z_f \sim q_\ph(\z_f \vert \x)}\left[ \log \frac{p(\x) }{p_\th(\x \vert \z_f))} \right]
\end{align}
\begin{align}
    \mathbb{E}_{\x \sim p(\x), \z_f \sim q_\ph(\z_f \vert \x)}\left[ \log p(\x) - \log p_\th(\x \vert \z_f)) \right]
\end{align}
which is dependent on the reconstruction loss. The dependence on $q_\ph(\z_f \vert \x)$ implies that tighter correlation between $\z_f$ and $\x$ means a larger channel capacity. Due to the increase in  variance of $q_\ph(\z_f \vert \x)$ for increasing temperature, the channel capacity decreases with temperature. 
\begin{align}
    \mathbb{E}_{\x \sim p(\x), \z_f \sim q_\ph(\z_f \vert \x)}\left[ \log p(\x)  - \log p_\th(\x \vert \z_f)) \right]
\end{align}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/Generative_Model_fig.png}
    \caption{a) A parameterized function $f_\theta : Z \rightarrow X$ from the metric space $(Z, d_Z)$ to the metric space $(X, d_X)$. Given three points $z_i, z_j, z_k \in Z$, $f_\theta$ is a map to $f_\theta(z_i), f_\theta(z_j), f_\theta(z_k) \in X$ such that the expectation over $d_Z(z_i, z_j)$ is $\epsilon$-close to $d_Z(f(z_i), f(z_j))$. b) Given $f_\theta$, we map $f_\theta(z_k)$ to a latent parameter for a probability distribution with support in $X$. Here, the probability distribution over $X$ is a Gaussian mixture model with mean and variance given by $f(z_j)$.}.
    \label{fig:isometry}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/Figure_Quadratic_Hamming.png}
    \caption{The quadratic Hamming metric on a $2 \times 2$ square lattice with excitation strings $z_a = \{1, 0, 0, 1\}$ and $z_b = \{1,0,1,0\}$. a) Shows a metric graph constructed by embedding the lattice sites into a 2D plane. Each site is assigned a position $v_i$ and the edge $d_V(v_i, v_j)$ is computing via the Euclidean distance $\vert v_i - v_j\vert ^2$ between sites. b) The excitation strings are imposed on the lattice sites (shaded sites are excited and correspond to a `$1$' in the string while unshaded sites are unexcited and correspond to a `$0$'). For each pair of excited lattice sites, }
    \label{fig:quad_Hamming}
\end{figure*}

Despite the theorized scaling advantage for these tasks, quantum computers suffer from two major roadblocks, decoherence due to noisy coupling with the outside environment and low qubit counts, both of which make solving real-world engineering problems impractical. 
Recent work in neutral atom quantum computing demonstrated breakthroughs in both qubit counts and coherence times by simulating quantum phases on a record 256 Rydberg atoms and impirically measuring scaling advantage for the MIS problem. While these breakthroughs show promise for future devices, we need algorithms that can mitigate both of these issues to apply quantum algorithms for practical engineering problems in the near-term, including the design of quantum computers themselves.
Each quantum computer has a native NP-Hard problem, determined by the choice of physical system, that can be optimized with no ancillary qubits, e.g. quadratic unconstrained binary optimization for quantum annealers and maximum independent set (MIS) for neutral atoms. 
Mapping other NP-Hard problems on quantum hardware is as simple as mapping one NP-Hard problem to the native NP-Hard problem via NP reductions, a very well studied idea in computational complexity theory.
However, mapping non-native optimization problems, i.e., optimization problems which do not natively map cleanly onto quantum hardware or for which a NP reduction is not known, has only recently been possible through machine learning.
By training a binary variational autoencoder, sampled solutions of a non-native problem, e.g., material shape design, can be mapped onto quantum pure states and an objective function can be constructed through Hamiltonian learning.
While this technique shows practical performance improvements for optimization tasks over other machine learning assisted optimization algorithms, it did not consider the native quantum Hamiltonian as a part of the training process, and instead used a simple Gumbel-Softmax reparameteriation trick to sample the latent space.
This is because training a quantum variational autoencoder requires computing the gradient of the probability distribution generated by the quantum computer, i.e., the quantum gradient.
Computing the quantum gradient is difficult in practice due to the magnitude of the gradient being over-whelmed with noise, also known as the Barren Plateu problem. Drawing inspiration from the classical setting, adversarial autoencoders solve several issues with computing the gradient of the Kullback-Liebler Divergence term found in the evidence lower bound of variational autoencoders, which is where the quantum gradient calculation takes place.
If the KL-divergence term doesn’t have a clean, samplable closed-form gradient, then it must be approximated with high variance.
Therefore, adversarial autoencoders replace this term with an ad-hoc discriminator loss to regularize the encoder’s distribution with the chosen prior. Furthering the use of classical advancements, by introducing a gradual noising schedule in the latent space of the autoencoder, denoising diffusion models achieve state-of-the-art performance for generating samples from the engineering design space.
Taking inspiration from the denoising diffusion models, we introduce a quantum adversarial  diffusion model trained on a Rydberg atom quantum simulator. We consider the problem of designing a metalens for trapping Rydberg atoms, an engineering design problem that will improve the quality of the neutral atom simulator used for sampling, thereby demonstrating the first instance of a quantum computer sampling new designs for itself and performing quantum bootstrapping.

